The Integration of Machine Learning into Automated Test Generation: A Systematic Mapping Study

Context: Machine learning (ML) may enable effective automated test generation. Objective: We characterize emerging research, examining testing practices, researcher goals, ML techniques applied, evaluation, and challenges. Methods: We perform a systematic mapping on a sample of 124 publications. Results: ML generates input for system, GUI, unit, performance, and combinatorial testing or improves the performance of existing generation methods. ML is also used to generate test verdicts, property-based, and expected output oracles. Supervised learning - often based on neural networks - and reinforcement learning - often based on Q-learning - are common, and some publications also employ unsupervised or semi-supervised learning. (Semi-/Un-)Supervised approaches are evaluated using both traditional testing metrics and ML-related metrics (e.g., accuracy), while reinforcement learning is often evaluated using testing metrics tied to the reward function. Conclusion: Work-to-date shows great promise, but there are open challenges regarding training data, retraining, scalability, evaluation complexity, ML algorithms employed - and how they are applied - benchmarks, and replicability. Our findings can serve as a roadmap and inspiration for researchers in this field.

==> old_text_results.tex <==
\subsubsection{GUI Test Generation}

GUI testing is a form of system testing focused specifically on testing through the graphical user interface of an application. This form of testing can be used to verify functionality, but can also focus on elements unique to the interface, such as inconsistent font, color, iconography, or other graphical elements or broken links. To properly test software through the GUI, one must explore the interface with the hopes of triggering a failure. To guide this exploration, the publications in this area (see Table~\ref{tab:GUIresults}) often portray the interface as a state machine, and model changes to the on-screen display as transitions taken through actions applied in the GUI. The goal of test generation is often to arrive at the highest possible number of unique states. Of the \papersgui publications in this pool, eleven focus on mobile applications, four focus on web applications, and two on desktop applications.

Ten contributions focusing on mobile applications have used ML to guide the search for unvisited states, while one tried to find violations of specifications written in a temporal logic. Almost all of these publications adopted a RL technique to guide exploration. This recurrent adoption of RL-based approaches occurs because GUI exploration is handled in sequential steps, giving the algorithm time to analyze the current state and take actions likely to cover new states. The most commonly used RL technique in this area is Q-learning~\cite{Vuong2018,Mariani2012,Koroglu2018,Adamo2018, Yasin2021, Brunetto2021, Yasin2021, Zheng2021a}. Q-learning associates the value of an action with particular states or types of state. It can account for stochastic transitions and does not require a pre-existing model of the environment/SUT. During navigation, Q-learning uses the same function to evaluate the reward from both the actual and projected actions. In noisy environments, this can exaggerate estimations of the value of future actions, misleading the exploration. Double Q-learning, as used by Koroglu and Sen~\cite{Koroglu2020,Koroglu2021}, attempts to correct this issue by using a different equation to calculate future rewards. Collins et al.~\cite{Collins2021} adopted a deep convolutional neural network to guide the RL agent,referred to as a Deep Q-Network. 

The main difference between these publications lies in how the reward associated with an action is determined. The reward function determines which actions are chosen, when they are chosen, and how often they are chosen. Thus, it has a major role to play in determining the effectiveness of test generation. 

Many of the publications base the reward function in part on the state coverage (e.g.,~\cite{Yasin2021}), while also incorporating additional information to bias the selection of states. Collins et al. rewarded exploration by assessing the magnitude of the change in state, with large changes (e.g., transitioning to a new activity) being rewarded more heavily. 
Koroglu et al. incorporate usage specifications and expectations into the reward function~\cite{Koroglu2018,Koroglu2020}. This also allows the RL approach to serve as a form of oracle to judge the correctness of the app under test. Mathematically representing these requirements is a task assigned to humans.  
Mariani et al. extend state coverage by also giving a reward for each unique function~\cite{Mariani2012}.
Pan extends state coverage by incorporating a curiosity factor, which changes the reward depending on the number of times the RL agent interacts with each element~\cite{Pan2020}. Degott et al. consider not just the elements that can be interacted with, but also the interaction possibilities that exist for each element (e.g. click, double click, drag, hold)~\cite{Degott2019}. The RL agent must learn how to interact with the elements, rather than relying on predefined instructions like in other publications. This increases the complexity of the learning task and increases the required computational overhead of performing RL, but improves applicability of the approach. 

In recent work, Koroglu and Sen~\cite{Koroglu2021} use specifications written in a formal logic as the basis of the reward function. Test cases that come closer to violating these specification statements are rewarded more heavily. 

If the app GUI has a ``home'' or ``back'' button, loops are created in navigation of the GUI. This can prove challenging for ML approaches, leading to wasted effort trapped in these loops. With this in mind, Choi et al. aim to minimize testing time by identifying and exploiting these loop closures, resulting in a faster learning rate while also avoiding restarting the app~\cite{Choi2013a}.

Only one approach targeted mobile applications using supervised learning~\cite{Li2019}, using it to mimic human interaction based on recorded logs of user interactions with the SUT. The authors used a Deep Neural Network (DNN), a complex form of NN with several hidden layers. This architecture enables the NN to achieve more accurate results at the cost of consuming more computational resources and processing time. The intent is that the DNN will be capable of replicating the same actions as a real user, and the authors use accuracy as a measure to validate the trained model. The test generation framework is evaluated using the state coverage. The DNN associates GUI elements with a probability of usage by a human, using those probabilities to bias the selection of actions. However, a limitation is that using previously-labelled probabilities might lead the framework to always make the same choices and cycle through the same states. With this problem in mind, the authors plan to explore RL-based approaches in future work. 

The majority of the Mobile App GUI test generation frameworks evaluate effectiveness by measuring the achieved state coverage. Koroglu and Sen~\cite{Koroglu2021} also evaluate based on the number of faults detected. Collins et al~\cite{Collins2021} and Yasen et al.~\cite{Yasin2021} evaluate in terms of code coverage and crashes detected. These publications focus on Android apps from either the Play Store or the well-known F-Droid benchmark.

Santiago~\cite{Santiago2018,Santiago2019}, Kamal~\cite{Kamal2019}, and Zheng et al.~\cite{Zheng2021a} focus instead on web applications. Santiago uses supervised ML to generate input, while Kamal makes use of an unsupervised approach, and Zheng uses RL. Santiago focuses on generation of ``test flows''---sequences of events that can be performed against a web application. Their approach is trained using a set of human-written test flows spanning several webpages belonging to disparate domains. In both cases, the ML algorithm is validated by its accuracy in producing the same outputs as the data used for validation. Their first study uses a Recurrent Neural Network (RNN) to perform the learning task, and the test generation framework is evaluated using the achieved state coverage~\cite{Santiago2018}. 

Their second study extends the approach to interact with web forms by using Natural Language Processing (NLP) to extract information from feedback messages received when interacting with forms. The NLP framework then constructs constraints based on a series of rules, which are used to generate test input through a standard constraint solver. A Random Forest classification is used to label web page components before applying the NLP framework. These labels help control how NLP is applied, as the application differs between different component types. This technique was evaluated by inserting mutants---synthetic faults---into the GUI, where the number of mutants detected servers as the evaluation metric. Their approach could, potentially, be faster and more accurate than a RL-based approach. However, it requires a time-consuming and data-dependent training phase and a sizeable set of human-created input. Santiago claims that the models trained in can be used for multiple websites, decreasing the training burden. 

Kamal et al. propose a framework that identifies GUI elements from the source code, then uses two search-based approaches to generate input for the page~\cite{Kamal2019}. The first algorithm creates test input based on the GUI's most rewarded action for the current state. The second produces sequences of input data that could lead to new states. ML is used to eliminate redundant test cases. The ML approach used is a Feedforward Artificial Neural Network (ANN)---a simplistic type of NN, with no cycles or loops in the neurons' connections. It learns a model associating input to output, and uses the predicted output to decide if one test is redundant to another. The state coverage is used to evaluate the framework.

Zheng et al.~\cite{Zheng2021a} use a RL-based approach to explore a state-based model of a web application. Their approach uses Q-Learning, with a reward function based on rewarding curiosity---updating the probability of selecting a state transition to explore based on the state coverage of earlier actions. They evaluate their approach in terms of achieved code coverage, fault detection, and scalability on a large number of web apps. Their evaluation is over a research benchmark used in prior work, 50 real-world web apps, and an industrial Software as a Service system. 
Brunetto et al.~\cite{Brunetto2021} reported on using a RL-based GUI test generation tool in an industrial environment. Their approach was based on Q-Learning, and rewarded state coverage. They evaluated their approach qualitatively on an enterprise resource planning application, explaining the challenges encountered in practice and the improvements made following feedback from developers.

Ariyurek et al~\cite{Ariyurek2021} use RL to test 2D games. They apply two RL agent types---based on Monte Carlo Tree Search and Sarsa---to select movement actions for grid-based 2D games. The state of the game is represented as a graph, and ``test goals''---in the form of a modified game graph---are synthesized from the graph. The reward function emphasizes coverage of the test goal graph. The authors assess their framework based on the percentage of planted faults found in three games. 

Specifically for \textbf{GUI test generation}, we can answer RQ2-5 as follows:
\begin{itemize}
    \item \textbf{RQ2 (Goal of ML):}  ML is generally used to guide exploration of the GUI---often expressed in terms of states and transitions. ML may also generate a state-based model for use in generation or to filter redundant tests.
    \item \textbf{RQ3 (Integration of ML):} RL approaches often select interactions with the GUI from a set available in the current state, then receive feedback used to refine estimations on the actions that will increase coverage of a formulated state machine model. They may also attempt to violate specifications. Supervised techniques learn models of how state changes and generate new input sequences, and one technique is used to predict test redundancy. 
    \item \textbf{RQ4 (ML Techniques):} The most common approach is RL (83\% of publications, 15), in the form of Q-learning (59\%, 10), Deep Q-Networks, Monte Carlo Tree Search, and Sarsa. Supervised ML is also employed (22\%, 4 publications), based on various NNs and Random Forest. 
    \item \textbf{RQ5 (Evaluation of Approach):} The most used evaluation measurement for GUI test generation is state coverage (61\%, 11 publications). Other common metrics for evaluation are the number of faults or crashes detected (28\%, 5 publications), code coverage (11\%, 2), the number of mutants (synthetic faults) (6\%), and scalability (6\%).
\end{itemize}
